Sequential Fair Allocation of Limited Resources under Stochastic Demands

We consider the problem of dividing limited resources between a set of agents arriving sequentially with unknown (stochastic) utilities. Our goal is to find a fair allocation - one that is simultaneously Pareto-efficient and envy-free. When all utilities are known upfront, the above desiderata are simultaneously achievable (and efficiently computable) for a large class of utility functions. In a sequential setting, however, no policy can guarantee these desiderata simultaneously for all possible utility realizations. A natural online fair allocation objective is to minimize the deviation of each agent's final allocation from their fair allocation in hindsight. This translates into simultaneous guarantees for both Pareto-efficiency and envy-freeness. However, the resulting dynamic program has state-space which is exponential in the number of agents. We propose a simple policy, HopeOnline, that instead aims to `match' the ex-post fair allocation vector using the current available resources and `predicted' histogram of future utilities. We demonstrate the effectiveness of our policy compared to other heurstics on a dataset inspired by mobile food-bank allocations.

==> parts/ethics.tex <==
\section*{Ethics Statement}

Recent work in theoretical computer science and economics has been on designing markets that maximize `social good' without money~\cite{prendergast2017food}.  In these systems, instead of a primary objective of maximizing revenue, mechanism designers instead focus on maximizing some global value to society.  As an example, in school choice, researchers focus on designing matching schemes which satisfy capacity constraints at the school while ensuring that students are matched to a school high on their preference list~\cite{abdulkadirouglu2003school,abdulkadirouglu2005boston}.  In this setting, mechanism designers are more motivated in designing algorithms where students are placed at a school high on their preference, instead of focusing on each student having equal access to different schools (as not all students want to go to each school).  

However, other settings involves designing systems to allocate scarce resources when each agent has increasing utility with respect to the allocation received.  Common examples of this are in \cref{section: examples}, but include allocation of food to distribution sites in a food bank, hospital ICU beds and ventilator assignments, and processor assignment in cloud computing platforms~\cite{donahue2020fairness,ghodsi2011dominant}.  In these settings, designing allocations which maximize some form of `global social good' sacrifices individual fairness properties.  In food bank resource allocation, distribution sites are more concerned in receiving a fair share of the allocation instead of maximizing social good of the entire system. 

In our research, we focus on designing online allocation algorithms which give \emph{individual} instead of global fairness guarantees.  Algorithms of this form necessarily sacrifice global properties to benefit the individuals.  Through \cref{sec:experiments} we show that our algorithm \HopeOnline improves on several benchmarks with respect to fairness metrics applied to several datasets motivated by our local food-bank.  Our algorithm helps inform policy decisions on the food-bank level by showing how to balance individual fairness guarantees across the different distribution sites.

Implementing these algorithms in practice could have unforeseen consequences.  In particular, by focusing on generating individual guarantees the allocations necessarily sacrifice global properties (not necessarily using up all available resources, etc).  Stakeholders interested in using these algorithms in practice should use offline experiments with available data to ensure allocations produced match their goals.  For further discussion on the model see \cref{app:varian}.
